Science-Driven Tunable Design of Cosmic Explorer Detectors

Ground-based gravitational-wave detectors like Cosmic Explorer can be tuned to improve their sensitivity at high or low frequencies by tuning the response of the signal extraction cavity. Enhanced sensitivity above 2 kHz enables measurements of the post-merger gravitational-wave spectrum from binary neutron star mergers, which depends critically on the unknown equation of state of hot, ultra-dense matter. Improved sensitivity below 500 Hz favors precision tests of extreme gravity with black hole ringdown signals and improves the detection prospects while facilitating an improved measurement of source properties for compact binary inspirals at cosmological distances. At intermediate frequencies, a more sensitive detector can better measure the tidal properties of neutron stars. We present and characterize the performance of tuned Cosmic Explorer configurations that are designed to optimize detections across different astrophysical source populations. These tuning options give Cosmic Explorer the flexibility to target a diverse set of science goals with the same detector infrastructure. We find that a 40 km Cosmic Explorer detector outperforms a 20 km in all key science goals other than access to post-merger physics. This suggests that Cosmic Explorer should include at least one 40 km facility.

==> Makefile <==
# Usage
#
# compile the document
# 	make

# clean the directory
#	make clean
#
# make a marked up pdf showing changes from the last version
#	make diff
#
# make a marked up pdf showing changes from v2
#	make diff REV=v2
#
# make a marked up pdf showing changes from commit 34ffa8f82f1b033567979533beba2ad18ab349a8
#	make diff REV=34ffa8f82f1b033567979533beba2ad18ab349a8

.PHONY: all tex clean diff

DOC = main
REV = v1

ifeq ($(REV), v2)
	COMMIT = 050db08faa60096be0d4bf7f824bce8eee2f1160
else ifeq ($(REV), v1)
	COMMIT = 99401778173d0a78af2aee8de1b477d7880dda67
else
	COMMIT = $(REV)
endif

all: tex

tex:
	latexmk -pdf $(DOC).tex

clean:
	latexmk -c
	rm -f *.aux
	rm -f *.bbl

diff: tex
	git latexdiff --flatten --config="PICTUREENV=(?:picture|DIFnomarkup|tabular|tblr)[\w\d*@]*" --ignore-latex-errors --no-view --main $(DOC).tex -o $(REV)_diff.pdf $(COMMIT)

